An Extension of Linear-size Suffix Tries for Parameterized Strings

In this paper, we propose a new indexing structure for parameterized strings which we call PLSTs, by generalizing linear-size suffix tries for ordinary strings. Two parameterized strings are said to match if there is a bijection on the symbol set that makes the two coincide. PLSTs are applicable to the parameterized pattern matching problem, which is to decide whether the input parameterized text has a substring that matches the input parameterized pattern. The size of PLSTs is linear in the text size, with which our algorithm solves the parameterized pattern matching problem in linear time in the pattern size. PLSTs can be seen as a compacted version of parameterized suffix tries and a combination of linear-size suffix tries and parameterized suffix trees. We experimentally show that PLSTs are more space efficient than parameterized suffix trees for highly repetitive strings.

==> docs/algo/algo_s2.tex <==
\begin{algorithm2e}[!h]
\caption{Simple p-matching algorithm ($\textsc{P-Match}(p, i,j, u)$)}
\label{alg:simplematch}
\KwIn{A string $p$, positions $i,j$ of $p$, and a node $u$ in $\PLST(T)$}
\KwOut{The highest descendant $v$ of $u$ such that $p[i:j]$ is a prefix of $\Label(u,v)$}
\If{$i > j$}{
	\Return $u$\;
}\Else{
	\If{$\Child_{\PLST}(u, p[i])$ is undefined}{
		\Return $\mathsf{Null}$\;
	}\Else{
		$v \leftarrow \Child_{\PLST}(u, p[i])$\;
		$l \leftarrow \min\{|p|,|v|-|u|\}$\;
		\If{$l \ge 2$}{
			\If{$1 \le \Recode(v) \le |p|$}{
				\If{$p[i+\Recode(v)-1] = |u| + \Recode(v) - 1$}{
					$p[i+\Recode(v)-1] \leftarrow 0$\;
				}\Else{
					\Return $\mathsf{Null}$\;
				}
			}
			\If{$\textsc{P-Match}(p,i,i+l-1,\Slink(u)) = \mathsf{Null}$}{
				\Return $\mathsf{Null}$\;
			}
		}
	}
	\Return $\textsc{P-Match}(p,i+l,j,v)$\;
}
\end{algorithm2e}

==> docs/algo/edge_check_algo.tex <==
\begin{algorithm2e}[!h]
\caption{Checking edge algorithm for PLST ($\textsc{EdgeCheck}(p, (u, v))$)}
\label{alg:edge_check_algo}
\KwIn{A string $p$ and an edge $(u, v)$ in $\PLST(T)$}
\KwOut{Whether $p$ matches a prefix of $\Label_{\PSTrie}(u, v)$}
%\If{$\Child_{\PLST}(u, p[1])$ is defined}{
%	$v \leftarrow \Child_{\PLST}(u, p[1])$\;
%}
%\Else{
%	\textbf{return} $False$\;
%}
\If{$|v| - |u| = 1$}{
	%$p \leftarrow p[2:|p|]$\;
	\Return \textsf{True}\;
}
\Else{
	\If{$\Recode(v) \neq 0$ \emph{ and }$\Recode(v) \leq |p|$}{
		\If{$p[\Recode(v)] = \Recode(v) + |u| - 1$}{
			$p[\Recode(v)] \leftarrow 0$\;
		}
		\Else{
			\Return \textsf{False}\;	
		}			
	}
	$z \leftarrow \Slink(u)$\;	
	\While{$p \neq \epsilon$}{
		\If{$\Child(z, p[1])$ is defined}{
			$z^\prime \leftarrow \Child(z, p[1])$\;
		}
		\Else{
			\Return \textsf{False}\;
		}
		$l \leftarrow \min\{|p|,|z'| - |z|\}$\;
		\If{$\textsc{EdgeCheck}(p[1 : l], (z, z')) = \mathsf{True}$}{
			$p \leftarrow p[l + 1:|p|]$\;
			$z \leftarrow z^\prime$\;
		}
		\Else{
			\Return \textsf{False}\;
		}
	}
	\Return \textsf{True}\;
}
\end{algorithm2e}

==> docs/algo/para_match_algo.tex <==
\begin{algorithm2e}[!h]
\caption{Parameterized pattern matching algorithm with PLST ($\textsc{P-Match}(p)$)}
\label{alg:PARA_MATCH}
\KwIn{Pattern $p = \pre{P}$}
\KwOut{The set of position $i$ such that $T[i:i+|P|-1]\approx P$}

$u \leftarrow \text{ the root}$\;
\While{$p \neq \epsilon$}{
	%\If{$p$ = $\epsilon$}{
	%	{\bf return} $u$\;
	%}
	%\Else{
		\If{$\Child(u, p[1])$ is undefined}{
			\Return $\emptyset$\;
		}
		\Else{
			$v \leftarrow \Child(u, p[1])$\;
			$l \leftarrow \min(|p|, |v| - |u|)$\;
			\If{$\textsc{EdgeCheck}(p[1:l], (u, v)) = \mathsf{True}$}{
				%$P \leftarrow p[l + 1:|p|]$\;
				$u \leftarrow v$\;
				$p \leftarrow p[l + 1:|p|]$\;
			}
			\Else{
				\Return $\emptyset$\;
			}
		}
	%}
}
\Return the indices of the leaves that have $u$ as an ancestor\;
% $\{\mbox{leaf number of } v | \mbox{ leaf node } v \mbox{ s.t. } u  \mbox{ is an ancestor node of }v \}$\;
\end{algorithm2e}

==> docs/macro.tex <==
%#! platex main

%Packages --------------------------------------------------
%\usepackage{amssymb}
\usepackage{amsmath}
%\usepackage{amsthm}
%\usepackage{graphicx}
%\usepackage{multirow}
%\usepackage{colortbl}
%\usepackage[rightcaption]{sidecap}



\usepackage[algoruled,linesnumbered,algo2e,lined,noend]{algorithm2e}
\usepackage{comment}
\usepackage{hyperref}
\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage{color}
%\newtheorem*{lem}{Lemma}
\spnewtheorem{observation}{Observation}{\bfseries}{\itshape}


\newcommand{\shinocom}[1]{\textcolor{magenta}{[(ayumi) #1]}}
\newcommand\nakashimacom[1]{{\color{blue}{[(nakashima): #1]}}}
\newcommand{\ryoshi}[1]{\textcolor{red}{[(ryo) #1]}}

\newcommand{\mi}[1]{\mathit{#1}}

\newcommand{\etal}{et al.}
\newcommand{\para}[1]{{#1}}
\newcommand{\set}[1]{{\bf{#1}}}
%\newcommand{\str}[1]{{{#1}}}
\newcommand{\str}[2]{{\mathsf{str}({#1},{#2}})}
\newcommand{\psufp}[1]{\mathit{psp}({#1})}
\newcommand{\pre}[1]{\mathsf{prev}({#1})}
\newcommand{\nex}[1]{\mathit{next}({#1})}
\newcommand{\occ}{\mathit{occ}}
\newcommand{\rt}{\mathit{root}}
\newcommand{\node}[1]{{#1}}
\newcommand{\descendant}[2]{\mathit{Des}_{#1}({#2})}
\newcommand{\zero}{\set{Z}}

\newcommand{\calN}{{\cal N}}

\newcommand{\primary}[1]{\mathit{prim}(#1)}
\newcommand{\secondary}[1]{\mathit{sec}(#1)}

\newcommand{\actn}{\mathit{activenode}}
\newcommand{\newactn}{\mathit{newnode}}
\newcommand{\ans}{\mathit{ans}}

\newcommand{\child}[2]{\mathit{child}(#1,#2)}
\newcommand{\depth}[1]{\mathit{depth}(#1)}
\newcommand{\norm}[2]{\mathit{normalize}(#1,#2)}
\newcommand{\nll}{\textsf{null}}
\newcommand{\create}{\textsf{create}}

\newcommand{\return}{\mathbf{return}}


% add cpm2018
\newcommand{\STree}{\mathsf{STree}}
\newcommand{\STrie}{\mathsf{STrie}}
\newcommand{\LST}{\mathsf{LST}}
\newcommand{\PSTree}{\mathsf{PSTree}}
\newcommand{\PSTrie}{\mathsf{PSTrie}}
\newcommand{\Recode}{\mathsf{Re}}

\newcommand{\activeNode}{\mathit{activeNode}}
\newcommand{\linkNode}{\mathit{linkNode}}
\newcommand{\nextNode}{\mathit{nextNode}}
\newcommand{\Node}{\mathsf{node}}
\newcommand{\Root}{\mathit{root}}
\newcommand{\newLeaf}{\mathit{newLeaf}}
\newcommand{\Shrink}{\mathsf{sl}}
\newcommand{\Slink}{\mathsf{SL}}
\newcommand{\Flink}{\mathsf{FL}}
\newcommand{\Lcp}{\mathsf{lcp}}
\newcommand{\LCP}{\mathsf{LCP}}
\newcommand{\PLST}{\mathsf{PLST}}
\newcommand{\Tree}{\mathcal{T}}
\newcommand{\PTree}{\mathcal{P}}
\newcommand{\Dol}{\mathtt{\$}}
\newcommand{\Child}{\mathsf{child}}
\newcommand{\Depth}{\mathsf{depth}}
\newcommand{\Link}{\mathsf{link}}
\newcommand{\Rlink}{\mathsf{rlink}}
\newcommand{\Parent}{\mathsf{parent}}
\newcommand{\NULL}{\mathsf{NULL}}
\newcommand{\Plus}{\mathsf{+}}
\newcommand{\Type}{\mathsf{type}}
\newcommand{\Label}{\mathsf{lab}}
\newcommand{\PATH}{\mathsf{path}}
\newcommand{\True}{\mathsf{true}}
\newcommand{\False}{\mathsf{false}}
\newcommand{\Path}{\mathsf{plabel}}
\newcommand{\ot}{:=}
\newcommand{\Pair}[2]{\langle \mathtt{#1}, #2 \rangle}
\newcommand{\Ret}{\mathbf{return}}
\newcommand{\Stack}{\mathit{stack}}

\newcommand{\checkSuffixLink}{\mathsf{checkSuffixLink}}
\newcommand{\addLeaf}{\mathsf{addLeaf}}
\newcommand{\Leaf}{\mathit{leaf}}

\SetKwProg{Fn}{Function}{}{end}

%
\newcommand{\reencode}[1]{\langle #1 \rangle}
%\newcommand{\PSuff}{\mathsf{PrevSuff}}
\newcommand{\PSub}{\mathsf{PrevSub}}
\newcommand{\Diff}{\mathsf{diff}}
\newcommand{\vtx}[1]{#1}
%\newcommand{\vtx}[1]{[\![{#1}]\!]}




